Towards end-to-end verifiable online voting: adding verifiability to established voting systems

Online voting for independent elections is generally supported by trusted election providers. Typically these providers do not offer any way in which a voter can verify their vote, so the providers are trusted with ballot privacy and ensuring correctness. Despite the desire to offer online voting for political elections, this lack of transparency and verifiability is often seen as a significant barrier to the large-scale adoption of online elections. Adding verifiability to an online election increases transparency and integrity, allowing voters to verify that their vote has been recorded correctly and included in the tally. However, replacing existing online systems with those that provide verifiable voting requires new algorithms and code to be deployed, and this presents a significant business risk to commercial election providers. In this paper we present the first step in an incremental approach which minimises the business risk but demonstrates the advantages of verifiability, by developing an implementation of key elements of a Selene-based verifiability layer and adding it to an operational online voting system. Selene is a verifiable voting protocol that uses trackers to enable voters to confirm that their votes have been captured correctly while protecting voter anonymity. This results in a system where even the election authority running the system cannot change the result in an undetectable way, and gives stronger guarantees on the integrity of the election than were previously present. We explore the challenges presented by adding a verifiability layer to an operational system. We describe the results of two initial trials, which obtained that survey respondents found this form of verifiability easy to use and that they broadly appreciated it. We conclude by outlining the further steps in the road-map towards the deployment of a fully trustworthy online voting system.

==> authors.tex <==
%%%%%%%  JCS Format %%%%%%%%%


%\author[A]{\inits{N.}\fnms{Name1} \snm{Surname1}\ead[label=e1]{first@somewhere.com}%
%\thanks{Corresponding author. \printead{e1}.}},
%\author[B]{\inits{N.N.}\fnms{Name2 Name2} \snm{Surname2}\ead[label=e2]{second@somewhere.com}}
%and
%\author[B]{\inits{N.-N.}\fnms{Name3-Name3} \snm{Surname3}\ead[label=e3]{third@somewhere.com}}
%\runningauthor{N. Surname1 et al.}
%\address[A]{Department first, \orgname{University or Company name},
%Abbreviate US states, \cny{Country}\printead[presep={\\}]{e1}}
%\address[B]{Department first, \orgname{University or Company name},
%Abbreviate US states, \cny{Country}\printead[presep={\\}]{e2,e3}}


\author[A]{\fnms{Steve} \snm{Schneider}\ead[label=e1]{s.schneider@surrey.ac.uk}%
\thanks{Corresponding author. \printead{e1}.}} 
and
\author[A]{\fnms{Mohammed} \snm{Alsadi}\ead[label=e2]{m.alsadi@surrey.ac.uk}}
\runningauthor{S. Schneider et. al.}
\address[A]{Surrey Centre for Cyber Security, \orgname{University of Surrey}, \cny{UK} \printead[presep={\\}]{e1,e2}}
%\address[B]{Surrey Centre for Cyber Security, \orgname{University of Surrey}, \cny{UK} \printead[presep={\\}]{e2}}

%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%  IEEE Format %%%%%%%%%%%%%%

%\author{\IEEEauthorblockN{
%Mohammed Alsadi\IEEEauthorrefmark{1},
%Matthew Casey\IEEEauthorrefmark{2},
%Catalin Dragan\IEEEauthorrefmark{1},
%Fran\c{c}ois Dupressoir\IEEEauthorrefmark{3}
%Luke Riley\IEEEauthorrefmark{4} \\
%Muntadher Sallal\IEEEauthorrefmark{5}, 
%Steve Schneider\IEEEauthorrefmark{1},
%Helen Treharne\IEEEauthorrefmark{1}
%Joe Wadsworth\IEEEauthorrefmark{6}
%Phil Wright\IEEEauthorrefmark{7}} \\[2ex]
%
%\IEEEauthorblockA{\IEEEauthorrefmark{1}
%  Surrey Centre for Cyber Security,
%  University of Surrey, UK
%}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}
%  Pervasive Intelligence Ltd.
%} \\
%\IEEEauthorblockA{\IEEEauthorrefmark{3}
%  University of Bristol, UK
%}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}
%  Kings College London, UK
%}
%\IEEEauthorblockA{\IEEEauthorrefmark{5}
%  Nottingham Trent University, UK
%} \\
%\IEEEauthorblockA{\IEEEauthorrefmark{6}
%  formerly Electoral Reform Services Ltd.
%}
%\IEEEauthorblockA{\IEEEauthorrefmark{7}
%Civica Election Services Ltd.
%}}

==> configuration/packages.tex <==
\usepackage{comment}

\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{graphicx,rotating}
\usepackage{complexity}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{fix-cm}
\usepackage{courier}
\usepackage{listings}
\usepackage{subcaption}

\usepackage{multirow}

\usetikzlibrary{shadows}
\usetikzlibrary{shapes,positioning,arrows}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{shadows,arrows,patterns,automata,calc,intersections,fit,shapes.misc, decorations.markings}
\usepackage[underline=false,rounded corners=true]{pgf-umlsd}
\usepackage{todonotes}
\usepackage{paralist}
%\usepackage{parskip} % Creates paragraphs - Maybe remove for more space
\setdefaultenum{1)}{(a)}{i)}{A)}
\usepackage{multicol}% http://ctan.org/pkg/multicols
\usepackage{multirow}

% \usepackage[
% n,
% operators,
% advantage,
% sets,
% adversary,
% landau,
% probability,
% notions,
% logic,
% ff,
% mm,
% primitives,
% events,
% complexity,
% asymptotics,
% keys]{cryptocode}
\usepackage{dashbox}

\usepackage[
%pdfauthor={},
%pdfsubject={},
%pdftitle={},
%pdfkeywords={},
bookmarks=false,
breaklinks=true,
colorlinks=true,
linkcolor=black,
citecolor=black,
urlcolor=black,
%pdfstartpage=19,
pdfpagelayout=SinglePage
]{hyperref}
%enables correct jumping to figures when referencing
\usepackage[all]{hypcap}

\usepackage{dsfont}
\usepackage[bottom]{footmisc}
% \usepackage[nocompress]{cite}
\usepackage{listings}
\usepackage{fancyvrb}
\usepackage{bm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{cleveref}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{etoolbox}
\usepackage{varwidth} %for the varwidth minipage environment
\usepackage{array} % for defining a new column type
\usepackage{chngcntr}
\usepackage{stmaryrd}
\usepackage{tabulary}
\usepackage{booktabs}

\usepackage{wrapfig,epsfig}

\usepackage{xcolor}% http://ctan.org/pkg/xcolor
\usepackage{graphicx}
\usepackage{color}
\usepackage{todonotes}
% Fonts
\usepackage{microtype}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[utf8]{inputenc}
\usepackage{inconsolata}

\usepackage{enumitem}

%B-Method packages
% \usepackage{eventB}
% \usepackage{zed-csp}

% \usepackage[linesnumbered, ruled, noend]{algorithm2e} % algorithms
% \usepackage{algorithmicx}

\usepackage{float}
\usepackage{listing}
\usepackage{mdframed}
\usepackage{subcaption}
% \usepackage{draftwatermark}
% \SetWatermarkScale{1}


==> configuration/preamble.tex <==
% mark parts in an algoritm
\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}

\newcommand*{\AddNote}[4]{%
 \begin{tikzpicture}[overlay, remember picture]
  \draw [decoration={brace,amplitude=1.0em},decorate, thick]
  ($(#3)!(#1.north)!($(#3)-(0,1)$)$) --
  ($(#3)!(#2.south)!($(#3)-(0,1)$)$)
  node [align=center, text width=3.5cm, pos=0.5, anchor=west] {#4};
 \end{tikzpicture}
}

\makeatletter
\newcommand{\pushline}{\Indp}% Indent
\newcommand{\popline}{\Indm\dosemic}% Undent
\makeatother

\definecolor{mGray}{rgb}{0.0,0.0,0.0}
\lstdefinestyle{LemmaStyle}{
    numberstyle=\tiny\color{mGray},
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=1,
    basicstyle=\ttfamily\footnotesize,
    xleftmargin=2em,
}

% restyle matrix
\let\bbordermatrix\bordermatrix
\patchcmd{\bbordermatrix}{8.75}{4.75}{}{}
\patchcmd{\bbordermatrix}{\left(}{\left[}{}{}
\patchcmd{\bbordermatrix}{\right)}{\right]}{}{}

\let\abordermatrix\bordermatrix
\patchcmd{\abordermatrix}{8.75}{4.75}{}{}
\patchcmd{\abordermatrix}{\left(}{\left\langle}{}{}
\patchcmd{\abordermatrix}{\right)}{\right\rangle}{}{}
\usepackage{etoolbox}

% break (newline) on a comma in math mode
\AtBeginDocument{%
 \mathchardef\mathcomma\mathcode`\,
 \mathcode`\,="8000
}
{\catcode`,=\active
 \gdef,{\mathcomma\discretionary{}{}{}}
}

\newcolumntype{M}{>{\begin{varwidth}{1.5cm}}l<{\end{varwidth}}} %M is for Maximal column
\setlength\extrarowheight{2pt} % or whatever amount is appropriate

\newenvironment{tagcases}[1][]
{\empheq[left={#1\empheqlbrace}]{alignat=2}}
{\endempheq}

\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother

% sub cases in proofs
% \counterwithin*{equation}{definition}
\theoremstyle{remark}
\newtheorem{mycase}{Case}
\newtheorem{msgtheory}{Equation}
\theoremstyle{remark}
\newtheorem{mysubcase}{Case}
\numberwithin{mysubcase}{mycase}

% Example environment
\theoremstyle{definition}
\newtheorem{example}{Example}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\definecolor{bluekeywords}{rgb}{0.13,0.13,1}
\definecolor{greencomments}{rgb}{0,0.5,0}
\definecolor{redstrings}{rgb}{0.9,0,0}

\lstdefinestyle{tamarinStyle}{
 showspaces=false,
 showtabs=false,
 breaklines=true,
 showstringspaces=false,
 breakatwhitespace=true,
 escapeinside={(*@}{@*)},
 basicstyle=\footnotesize\ttfamily,
 breakatwhitespace=false,
 breaklines=true,
 captionpos=b,
 keepspaces=true,
 showspaces=false,
 showstringspaces=false,
 showtabs=false,
 tabsize=2
}

\lstset{style=tamarinStyle}

\restylefloat{figure}

\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefalias{AlgoLine}{line}
\makeatletter
\let\cref@old@stepcounter\stepcounter
\def\stepcounter#1{%
 \cref@old@stepcounter{#1}%
 \cref@constructprefix{#1}{\cref@result}%
 \@ifundefined{cref@#1@alias}%
 {\def\@tempa{#1}}%
 {\def\@tempa{\csname cref@#1@alias\endcsname}}%
 \protected@edef\cref@currentlabel{%
  [\@tempa][\arabic{#1}][\cref@result]%
  \csname p@#1\endcsname\csname the#1\endcsname}}
\makeatother


==> sec-evaluation.tex <==
\section{Trials}\label{sec:evaluation}

The system was deployed in April 2019, with 4 Verificatum nodes and 4 Quorum nodes.  In each case the threshold was 3 (i.e. greater than two thirds), meaning that three nodes were reuqired to cooperate to achieve consensus and function correctly.  CES ran two Verificatum nodes and two Quorum nodes at distinct geographic locations.  This was chosen to be below the threshold of 3 in order to ensure that CES did not possess sole control over the Verificatum or Quorum networks. However, the control of 2 nodes in each case meant that CES involvement was required to run the Verificatum and Quorum components and could not be excluded by a threshold of other parties.  The University of Surrey (UoS) ran one Verificatum node and one Quorum node on the Surrey campus, and ran a second one on the AWS server that was also hosting the vote verification website.

The first use of the system was with an in-house trial run of the system within Civica. This was followed by a second deployment to run the June 2019 student representatives election within the Department of Computer Science at the University of Surrey.  In both cases voters were able to verify their vote and to complete our initial questionnaire.  As a result of these two trials the system was tuned to make election setup easier, and the VMV website was simplified following voter feedback.  We also tuned the questionnaire.

The system was then used in two binding commercial ballots run by CES: a ballot in August 2019 to elect a West Midlands representative for the Royal College of Nursing, and a ballot to elect two representatives for the College of Podiatrists in October 2019. Both of these ballots were open for a period of several weeks, and in both cases the voters were invited to verify their vote after the close of the ballot, and to complete the questionnaire. The full questionnaire is given in Appendix~\ref{sec:questionnaire}.

For the initial trial, the electorate consisted of employees within a section of Civica, together with members of the project team.  The ballot asked voters to select one of a list of four chocolate bars, and the ballot was open for a week.  Following the close of the ballot, voters were offered the opportunity to verify their vote.  Those that followed the link to the verification page were then given the opportunity to complete the questionnaire.  In this ballot there were 136 votes cast, and there were 39 questionnaires started (36 completed), a proportion of 29\%.  We did not explicitly record the number of verifications performed but the requirement to verify before reaching the questionnaire gives a minimum verification rate of 29\%.

The student representatives trial consisted of two races for student representative (one for each programme), with two candidates in each race. The electorate consisted of students in a particular year on one of the degree courses that was electing a representative. Voters could only vote in the race appropriate to their degree course. In this trial there were 21 votes cast, and three questionnaires.  Although the numbers were small, this deployment was the first one external to CES and provided the confidence and feedback required to scale up to the two full trials.

The Royal College of Nursing ballot was a race between two candidates, with voters asked to select one candaidate.  The electorate consisted of members of the Royal College of Nursing within the West Midlands region. There were 942 votes cast, and 503 verification checks, a verification rate of 53\%.  Of those who verified, there were 162 completed questionnaires: 17\% of those who voted.

The College of Podiatrists ballot was conducted to select two representatvies from 6 candidates.  The electorate consisted of members of the College of Podiatrists.  Voters were asked to select two candidates from the list.  In this ballot there were 315 ballots cast, and 148 verification checks were carried out, a rate of 47\%.  There were 32 questionnaires completed: 10\% of those who voted.  


\begin{table*}[t]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
& \parbox[b]{1cm}{Strongly Disagree} 
& {Disagree} 
& \parbox[b]{1cm}{Weakly Disagree}
& \parbox[b]{0.8cm}{Weakly Agree} 
& {Agree} 
& \parbox[b]{0.8cm}{Strongly Agree} 
& \parbox[b]{1.1cm}{Responses} \\ \hline
\parbox{8cm}{Checking my vote gave me confidence that the election result is correct} & 2\% & 7\% & 7 \% & 22\% & 37\% & 26\% & N=192 \\ \hline
\parbox{8cm}{With this system I can tell how a particular person has voted} & 33\% & 46\% & 9 \% & 5\% & 3\% & 4\% & N=183 \\ \hline
\end{tabular}
\caption{Responses to selected questions} \label{table:questionnaire}
\end{center}
\end{table*}



The questionnaires were deployed "in the wild" on voters in a real binding ballot. The advantage of this approach is that we obtain responses from voters who are in exactly the situation where the system is intended to be used. However it must be borne in mind that the questionnaire was offered only to those voters who had verified their vote.  The opportunity to complete the questionnaire was therefore restricted to voters already engaged with the verification process.  This was necessary since the questionnaire is seeking feedback about the verification experience, however it is likely to bias the sample, since those that dislike technology or electronic voting are less likely to reach this stage.  The alternative would have been to carry out a ballot in a lab situation where participants are asked to carry out voting and verification tasks and then complete the questionnaire.  While this would allow for more control over obtaining a cross section of voters, the responses might not reflect how the voters would feel in a meaningful ballot.

Voters were generally happy with the opportunity to check their vote, and with the ease of doing so, and did not feel that the system was complicated.  Furthermore 85\% agreed with the statement that "Checking my vote gave me confidence that the election result is correct".  The full breakdown of answers for this question is given in Table~\ref{table:questionnaire}).
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.45\textwidth]{ERSTrials/QuestionnairePieGraphs/Slide7.jpg}
%\end{center}
%\caption{Questionnaire: Question 6} \label{questionnaire:qn6}
%\end{figure}
Despite these positive findings, our questions concering the voters' comprehension of and attitude to verifiability obtained more contradictory results that are difficult to interpret.  We had 42\% agreeing with the statement that "I don't see the point of checking my vote", and 80\% agreeing that they "wouldn't usually bother with checking [my] vote", but conversely 67\% agreed that they would check their vote next time if they could, and 72\% agreed that everyone should check their vote if the facility is available.

Finally with respect to privacy, the majority of voters recognised that the system did not reveal how a voter has voted. 84\% agreed that the checking system kept their vote private, 86\% agreed that other people could not tell which vote was theirs, and 88\% disagreed with the statement that they could tell how a particular person has voted (see Table~\ref{table:questionnaire}.  While these results are encouraging (since our hope is that voters will recognise that privacy is indeed provided), we must take care not to read too much into the results, since they provide the immediate reaction of voters on the basis of the interaction they have just had with it.  These voters are unlikely to have explored the list of all trackers against votes cast.  Exploration of voters' comprehension of the vote privacy provided by the system would ideally involve semi-structured intervews with voters around a fuller explanation of the system.
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.45\textwidth]{ERSTrials/QuestionnairePieGraphs/Slide15.jpg}
%\end{center}
%\caption{Questionnaire: Question 14} \label{questionnaire:qn14}
%\end{figure}

In addition to the questionnaire responses, we also provided an opportunity to provide some freeform comments on any aspect of the system that the voter wanted to provide.  This has provided qualitative feedback giving the broad range of voters' responses to the system.  

There were many positive comments around ease of use and confirming the vote, for example:
\begin{quote}
\emph{"Was easy and nice to know it was correct"} 
\end{quote}
\begin{quote}
\emph{"Very easy to use and reassuring that vote registered as I voted"}
\end{quote}
\begin{quote}
\emph{"I like and appreciate the opportunity to check my vote. In something as seemingly trustworthy as an RCN election it is a bonus. If I were voting in a General Election I would regard it as a necessity."} 
\end{quote}

Some respondents felt that the election authority should be trusted to ensure the system is secure and therefore there should be no need for verifiability, or could not see the point of verifiability:
\begin{quote}
\emph{"It isn't something I would use. I would trust that an organisation such as yours would have a secure system"}
\end{quote}
\begin{quote}
\emph{"Very easy but I don't understand the need to check. Do you feel that we don't trust the system ?"}
\end{quote}
\begin{quote}
\emph{"I don't see the point! Sorry! Once my vote is cast I assume it has been correctly processed or there are issues with the system. It tells me nothing about the robustness of the system and is a step that I would find not worthy of my time."} 
\end{quote}



Some respondents considered the question around privacy more deeply and identified some issues that would need to be answered for voters:
\begin{quote}
\emph{"Since there seems to be a permanent record of how someone votes there is risk of breach of anonymity. I would prefer no record to be held."}
\end{quote}
\begin{quote}
\emph{"As this is the first time I have used the vote checking system, the privacy of my vote is purely on a trust basis relating to data protection."}
\end{quote}
\begin{quote}
\emph{"I have no idea if this system keeps my vote private and/or that others can see how I or other people have voted."}
\end{quote}








